CosmoMIA: Cosmic Web-based redshift space halo distribution

Modern galaxy surveys demand extensive survey volumes and resolutions surpassing current dark matter-only simulations' capabilities. To address this, many methods employ effective bias models on the dark matter field to approximate object counts on a grid. However, realistic catalogs necessitate specific coordinates and velocities for a comprehensive understanding of the Universe. In this research, we explore sub-grid modeling to create accurate catalogs, beginning with coarse grid number counts at resolutions of approximately $5.5\,h^{-1}\rm Mpc$ per side. These resolutions strike a balance between modeling nonlinear damping of baryon acoustic oscillations and facilitating large-volume simulations. Augmented Lagrangian Perturbation Theory (ALPT) is utilized to model the dark matter field and motions, replicating the clustering of a halo catalog derived from a massive simulation at $z=1.1$. Our approach involves four key stages: Tracer Assignment: Allocating dark matter particles to tracers based on grid cell counts, generating additional particles to address discrepancies. Attractor Identification: Defining attractors based on particle cosmic web environments, acting as gravitational focal points. Tracer Collapse: Guiding tracers towards attractors, simulating structure collapse. Redshift Space Distortions: Introducing redshift space distortions to simulated catalogs using ALPT and a random dispersion term. Results demonstrate accurate reproduction of monopoles and quadrupoles up to wave numbers of approximately $k=0.6\,h$ Mpc$^{-1}$. This method holds significant promise for galaxy surveys like DESI, EUCLID, and LSST, enhancing our understanding of the cosmos across scales.

==> second.tex <==
% \usepackage[usenames,dvipsnames]{pstricks}
% \usepackage{epsfig}
% \usepackage{pst-grad} % For gradients
% \usepackage{pst-plot} % For axes
% \usepackage[space]{grffile} % For spaces in paths
% \usepackage{etoolbox} % For spaces in paths
% \makeatletter % For spaces in paths
% \patchcmd\Gread@eps{\@inputcheck#1 }{\@inputcheck"#1"\relax}{}{}
% \makeatother
% 
\psscalebox{1.0 1.0} % Change this value to rescale the drawing.
{
\begin{pspicture}(0,-5.997386)(14.107156,5.997386)
\psbezier[linecolor=black, linewidth=0.04](4.9371552,-4.9991884)(5.737476,-4.6063623)(7.337476,-4.6063623)(8.241543,-4.997163747787477)
\psbezier[linecolor=black, linewidth=0.04](4.1571555,-3.1231637)(5.303964,-2.5231638)(7.7060914,-2.5231638)(8.957155,-3.1231637477874754)
\psbezier[linecolor=black, linewidth=0.04](3.4171555,-1.2764728)(5.2571554,-0.42316374)(7.8571553,-0.42316374)(9.717946,-1.2698546541794702)
\psbezier[linecolor=black, linewidth=0.04](2.6571555,0.5768362)(5.1571555,1.6768363)(8.157155,1.5768362)(10.457155,0.5768362522125244)
\psbezier[linecolor=black, linewidth=0.04](1.8571554,2.5768363)(4.718025,3.7768362)(8.600634,3.6768363)(11.257155,2.5768362522125243)
\psbezier[linecolor=black, linewidth=0.04](8.228776,-4.9118752)(7.8512964,-5.902046)(11.49714,3.2558572)(11.929013,4.348156308580392)
\psbezier[linecolor=black, linewidth=0.04](1.1571555,4.3768363)(0.85715544,5.176836)(4.557921,-4.14038)(4.9100733,-5.019564009094422)
\psdots[linecolor=black, dotsize=0.2](6.767385,0.32185242)
\psdots[linecolor=black, fillstyle=solid, dotstyle=o, dotsize=0.2, fillcolor=white](8.096286,0.75944495)
\psbezier[linecolor=black, linewidth=0.04, arrowsize=0.04cm 2.0,arrowlength=0.8,arrowinset=2.0]{->}(6.8996215,0.44137785)(6.9738564,0.67683625)(7.3571553,0.87683624)(7.7886024,0.7905555165880651)
\psdots[linecolor=black, dotsize=0.2](4.265851,-0.5014246)
\psdots[linecolor=black, dotsize=0.2](9.565851,0.59857535)
\psbezier[linecolor=black, linewidth=0.04, arrowsize=0.04cm 2.0,arrowlength=0.8,arrowinset=2.0]{->}(4.325143,-0.7393802)(4.3777857,-1.0693631)(4.879789,-1.477902)(5.4584317,-1.3565698992625312)
\psdots[linecolor=black, fillstyle=solid, dotstyle=o, dotsize=0.2, fillcolor=white](5.796286,-1.3405551)
\psbezier[linecolor=black, linewidth=0.04, arrowsize=0.04cm 2.0,arrowlength=0.8,arrowinset=2.0]{->}(9.674252,0.7564923)(9.925294,1.1303986)(9.725304,1.4875665)(9.513972,1.5754410346296754)
\psdots[linecolor=black, fillstyle=solid, dotstyle=o, dotsize=0.2, fillcolor=white](9.196286,1.759445)
\psbezier[linecolor=black, linewidth=0.04](1.1571555,4.476836)(4.6571555,5.976836)(8.957155,5.676836)(11.957155,4.376836252212525)
\rput[bl](6.6071553,-0.15649708){\Large $\vec{s}$}
\rput[bl](8.007155,0.14350292){\Large $\vec{q}$}
\rput[bl](2.5071554,1.8435029){\huge $b_k$}
\rput[bl](3.3071554,-0.15649708){\huge $b_j$}
\rput[bl](4.0071554,-1.9564971){\huge $b_i$}
\psbezier[linecolor=black, linewidth=0.04, arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.0]{->}(3.823822,-2.2231638)(2.9571555,-2.2231638)(2.5404887,-0.9398304)(3.0571554,-0.3231637477874756)
\psbezier[linecolor=black, linewidth=0.04, arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.0]{->}(3.023822,-0.32316375)(2.1571555,-0.32316375)(1.7404888,0.9601696)(2.2571554,1.5768362522125243)
\psbezier[linecolor=black, linewidth=0.04, arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.0]{->}(3.8571556,-2.2231638)(1.4015999,-2.2231638)(-0.0067334324,1.334731)(1.4571555,3.4768362522125242)
\rput[bl](11.307156,1.3435029){\Large $k=j+1$}
\rput[bl](10.507155,-0.5564971){\Large $j$}
\rput[bl](9.707155,-2.356497){\Large $i=j-1$}
\rput[bl](1.1071554,-3.156497){\Large 1}
\rput[bl](2.8071554,-4.8564973){\Large 0}
\rput[bl](0.40715545,-5.456497){\Large 2}
\rput{-359.67255}(-0.024774168,-0.0096365195){\psarc[linecolor=black, linewidth=0.04, dimen=outer, tbarsize=0.07055555cm 5.0,arrowsize=0.033cm 2.0,arrowlength=1.4,arrowinset=1.5]{|->}(1.6738222,-4.3398304){1.2833333}{0.0}{90.0}}
\rput{-237.51918}(-1.3956659,-7.9136686){\psarc[linecolor=black, linewidth=0.04, dimen=outer, tbarsize=0.07055555cm 5.0,arrowsize=0.033cm 2.0,arrowlength=1.4,arrowinset=1.5]{|->}(1.4738221,-4.3398304){1.2833333}{0.0}{90.0}}
\rput{-126.44237}(6.320184,-5.8900385){\psarc[linecolor=black, linewidth=0.04, dimen=outer, tbarsize=0.07055555cm 5.0,arrowsize=0.033cm 2.0,arrowlength=1.4,arrowinset=1.5]{|->}(1.6738222,-4.53983){1.2833333}{0.0}{90.0}}
\rput[bl](1.2071555,-4.556497){\huge +1}
\end{pspicture}
}


